Data Capsule: A New Paradigm for Automatic Compliance with Data Privacy Regulations

The increasing pace of data collection has led to increasing awareness of privacy risks, resulting in new data privacy regulations like General data Protection Regulation (GDPR). Such regulations are an important step, but automatic compliance checking is challenging. In this work, we present a new paradigm, Data Capsule, for automatic compliance checking of data privacy regulations in heterogeneous data processing infrastructures. Our key insight is to pair up a data subject's data with a policy governing how the data is processed. Specified in our formal policy language: PrivPolicy, the policy is created and provided by the data subject alongside the data, and is associated with the data throughout the life-cycle of data processing (e.g., data transformation by data processing systems, data aggregation of multiple data subjects' data). We introduce a solution for static enforcement of privacy policies based on the concept of residual policies, and present a novel algorithm based on abstract interpretation for deriving residual policies in PrivPolicy. Our solution ensures compliance automatically, and is designed for deployment alongside existing infrastructure. We also design and develop PrivGuard, a reference data capsule manager that implements all the functionalities of Data Capsule paradigm.

==> case_studies.tex <==
\section{Case Study: Protecting Health Records}

%% \begin{itemize}
%% \item STRIDE tool for cohort discovery (HIPAA)
%% \item Sharing posts with friends on a social network (GDPR / CCPA)
%% \item Advertising on a social network (GDPR / CCPA)
%% \item Calculating enrollment statistics at a university (FERPA)
%% \end{itemize}

We are currently in the preliminary stages of a collaborative case study to apply the data capsule paradigm in a medical study of menstrual data collected via mobile app. The goal of this study~\cite{Symul385054} and similar work~\cite{liu2018predicting,10.1093/emph/eoy018} is to demonstrate the use of mobile apps to assess menstrual health and fertility. Data capsules can allow study participants to submit their sensitive data in the context of a policy which protects its use.

The analyses used in this study include histograms of demographic information (e.g. age); statistics about observations (e.g. how many observations were made in the context of a participant intending to conceive a child); and statistics describing observations (e.g. amount of bleeding) by day of the cycle. The original study calculated these statistics using R programs that primarily encode count, mean, max, min, and percentile queries; we are currently working to support these queries in \system.

For such a study, we would expect data subjects to either accept or reject a formal policy which encodes a subset of HIPAA---namely, that only differentially private statistics based on personal health information will be used in the study, and that the data will not be used for any other purpose. Users who specify a more restrictive policy will effectively not be included in the study.


%% This section describes the use of \system to enforce the HIPAA regulations in the context of a research study conducted on menstrual data collected from hundreds of study participants.

%% \subsection{Data and Analysis Tasks}

%% \todo{describe the data and what questions the study wants to answer}

%% \subsection{Analysis Programs}

%% \todo{show examples of pandas programs answering the questions, and how the static analysis works}

%% \subsection{Policies \& Data Subject Experience}

%% \todo{talk about how data subjects might select subsets of hipaa clauses, and show example dashboards and the full data capsule graph}


